Upper-Confidence Bound for Channel Selection in LPWA Networks with Retransmissions

In this paper, we propose and evaluate different learning strategies based on Multi-Arm Bandit (MAB) algorithms. They allow Internet of Things (IoT) devices to improve their access to the network and their autonomy, while taking into account the impact of encountered radio collisions. For that end, several heuristics employing Upper-Confident Bound (UCB) algorithms are examined, to explore the contextual information provided by the number of retransmissions. Our results show that approaches based on UCB obtain a significant improvement in terms of successful transmission probabilities. Furthermore, it also reveals that a pure UCB channel access is as efficient as more sophisticated learning strategies.

==> Makefile <==
# Quick Makefile to compile easily the report (make pdf)
FILE = IEEE_WCNC__2019__Paper__BMBM
IN   = $(FILE).tex
OUT  = $(FILE).pdf

quick:	pdf
all:	clean pdf evince clean
pdf:	$(OUT)


.PHONY:	quick all pdf evince compress clean send_zamok latexstats lint proselint

.SUFFIXES:
.SUFFIXES: .md .tex .pdf

# Construction rules
.md.pdf:
	pandoc --verbose --include-in-header header.tex -s -t latex -o $@ $<
	-evince $@ >/dev/null 2>/dev/null &

.tex.pdf:
	pdflatex $<
	pdflatex $<
	# We have to include BibTeX
	+bibtex  $*
	pdflatex $<
	pdflatex $<
	-pdfinfo $@ | grep -v ':[ \t]\+no' | grep --color=always "^[A-Za-z ]\+:"
	-evince $@ >/dev/null 2>/dev/null &

# Utility for the PDF
evince:
	-evince $(OUT) &

compress:
	PDFCompress $(OUT)

# Cleaner
clean:
	-mv -vf *.fls *.fdb_latexmk *.ps *.dvi *.htoc *.tms *.tid *.lg *.log *.id[vx] *.vrb *.toc *.snm *.nav *.htmp *.aux *.tmp *.out *.haux *.hidx *.bbl *.blg *.brf *.lof *.ilg *.ind *.meta *.fdb_latexmk *.fls *.gz*busy* /tmp/ 2>/dev/null

# Sender
send_zamok:
	CP $(OUT) besson@zamok.crans.org:~/www/phd/articles/

# Linters!
latexstats:
	latexstats.sh $(IN)
	latexstats.sh $(IN) | sed -r "s:\x1B\[[0-9;]*[mK]::g" > latexstats.txt

lint:	write-good.sh write-good

proselint:
	time proselint $(IN) | tee proselint_report.txt

write-good:
	time write-good --no-passive --no-weasel --no-tooWordy --no-adverb $(IN) | tee writegood_report.txt

write-good.sh:
	time write-good.sh $(IN) | tee writegood_sh_report.txt

